Enhancement attacks in biomedical machine learning

The prevalence of machine learning in biomedical research is rapidly growing, yet the trustworthiness of such research is often overlooked. While some previous works have investigated the ability of adversarial attacks to degrade model performance in medical imaging, the ability to falsely improve performance via recently-developed "enhancement attacks" may be a greater threat to biomedical machine learning. In the spirit of developing attacks to better understand trustworthiness, we developed two techniques to drastically enhance prediction performance of classifiers with minimal changes to features: 1) general enhancement of prediction performance, and 2) enhancement of a particular method over another. Our enhancement framework falsely improved classifiers' accuracy from 50% to almost 100% while maintaining high feature similarities between original and enhanced data (Pearson's r's>0.99). Similarly, the method-specific enhancement framework was effective in falsely improving the performance of one method over another. For example, a simple neural network outperformed logistic regression by 17% on our enhanced dataset, although no performance differences were present in the original dataset. Crucially, the original and enhanced data were still similar (r=0.99). Our results demonstrate the feasibility of minor data manipulations to achieve any desired prediction performance, which presents an interesting ethical challenge for the future of biomedical machine learning. These findings emphasize the need for more robust data provenance tracking and other precautionary measures to ensure the integrity of biomedical machine learning research.

==> blank <==

@ARTICLE{Pedregosa2011-fe,
  title     = "Scikit-learn: Machine learning in Python",
  author    = "Pedregosa, Fabian and Varoquaux, Ga{\"e}l and Gramfort,
               Alexandre and Michel, Vincent and Thirion, Bertrand and Grisel,
               Olivier and Blondel, Mathieu and Prettenhofer, Peter and Weiss,
               Ron and Dubourg, Vincent and {Others}",
  journal   = "the Journal of machine Learning research",
  publisher = "JMLR. org",
  volume    =  12,
  pages     = "2825--2830",
  year      =  2011
}


@INPROCEEDINGS{Koh2017-en,
  title     = "Understanding Black-box Predictions via Influence Functions",
  booktitle = "Proceedings of the 34th International Conference on Machine
               Learning",
  author    = "Koh, Pang Wei and Liang, Percy",
  editor    = "Precup, Doina and Teh, Yee Whye",
  abstract  = "How can we explain the predictions of a black-box model? In this
               paper, we use influence functions --- a classic technique from
               robust statistics --- to trace a model's prediction through the
               learning algorithm and back to its training data, thereby
               identifying training points most responsible for a given
               prediction. To scale up influence functions to modern machine
               learning settings, we develop a simple, efficient implementation
               that requires only oracle access to gradients and Hessian-vector
               products. We show that even on non-convex and non-differentiable
               models where the theory breaks down, approximations to influence
               functions can still provide valuable information. On linear
               models and convolutional neural networks, we demonstrate that
               influence functions are useful for multiple purposes:
               understanding model behavior, debugging models, detecting
               dataset errors, and even creating visually-indistinguishable
               training-set attacks.",
  publisher = "PMLR",
  volume    =  70,
  pages     = "1885--1894",
  series    = "Proceedings of Machine Learning Research",
  year      =  2017
}


@ARTICLE{Biggio2018-ka,
  title    = "Wild patterns: Ten years after the rise of adversarial machine
              learning",
  author   = "Biggio, Battista and Roli, Fabio",
  abstract = "Learning-based pattern classifiers, including deep networks, have
              shown impressive performance in several application domains,
              ranging from computer vision to cybersecurity. However, it has
              also been shown that adversarial input perturbations carefully
              crafted either at training or at test time can easily subvert
              their predictions. The vulnerability of machine learning to such
              wild patterns (also referred to as adversarial examples), along
              with the design of suitable countermeasures, have been
              investigated in the research field of adversarial machine
              learning. In this work, we provide a thorough overview of the
              evolution of this research area over the last ten years and
              beyond, starting from pioneering, earlier work on the security of
              non-deep learning algorithms up to more recent work aimed to
              understand the security properties of deep learning algorithms,
              in the context of computer vision and cybersecurity tasks. We
              report interesting connections between these apparently-different
              lines of work, highlighting common misconceptions related to the
              security evaluation of machine-learning algorithms. We review the
              main threat models and attacks defined to this end, and discuss
              the main limitations of current work, along with the
              corresponding future challenges towards the design of more secure
              learning algorithms.",
  journal  = "Pattern Recognit.",
  volume   =  84,
  pages    = "317--331",
  month    =  dec,
  year     =  2018,
  keywords = "Adversarial machine learning; Evasion attacks; Poisoning attacks;
              Adversarial examples; Secure learning; Deep learning"
}


@UNPUBLISHED{Rosenblatt2021-re,
  title    = "Can we trust machine learning in {fMRI}? Simple adversarial
              attacks break connectome-based predictive models",
  author   = "Rosenblatt, Matthew and Rodriguez, Raimundo and Westwater,
              Margaret L and Horien, Corey and Greene, Abigail S and Constable,
              Robert T and Noble, Stephanie and Scheinost, Dustin",
  abstract = "Functional connectome-based predictive models continue to grow in
              popularity and predictive performance. As these models become
              more widely used, researchers have begun to question the idea of
              bias in the models, which is a crucial component of ethics in
              artificial intelligence. However, we show that model
              trustworthiness is a more important but vastly overlooked
              component of the ethics of functional connectome-based predictive
              models. In this work, we define ``trust'' as robustness to
              adversarial attacks, or data alterations designed to trick a
              model. We show that typical implementations of connectome-based
              models are untrustworthy and can easily be manipulated through
              adversarial attacks. We use classification of self-reported
              biological sex in three datasets (Adolescent Brain Cognitive
              Development Study, Human Connectome Project, and Philadelphia
              Neurodevelopmental Cohort) and for three types of predictive
              models (support vector machine (SVM), logistic regression, kernel
              SVM) as a benchmark to show that many forms of adversarial
              attacks are effective against connectome-based models. The
              attacks include changing the prediction by altering the data at
              test time, real-world changes at the time of scanning, and
              improving performance by injecting a pattern into the data.
              Despite drastic changes in prediction performance after
              adversarial attacks, the corrupted connectomes appear nearly
              identical to the original ones and perform similarly in
              downstream analyses. These findings demonstrate a need to
              evaluate the trustworthiness and ethics of connectome-based
              models before we can apply them broadly, as well as a need to
              develop methods that are robust to a wide range of adversarial
              attacks.",
  month    =  oct,
  year     =  2021
}


@INPROCEEDINGS{Munoz-Gonzalez2017-lg,
  title     = "Towards Poisoning of Deep Learning Algorithms with Back-gradient
               Optimization",
  booktitle = "Proceedings of the 10th {ACM} Workshop on Artificial
               Intelligence and Security",
  author    = "Mu{\~n}oz-Gonz{\'a}lez, Luis and Biggio, Battista and Demontis,
               Ambra and Paudice, Andrea and Wongrassamee, Vasin and Lupu, Emil
               C and Roli, Fabio",
  abstract  = "A number of online services nowadays rely upon machine learning
               to extract valuable information from data collected in the wild.
               This exposes learning algorithms to the threat of data
               poisoning, i.e., a coordinate attack in which a fraction of the
               training data is controlled by the attacker and manipulated to
               subvert the learning process. To date, these attacks have been
               devised only against a limited class of binary learning
               algorithms, due to the inherent complexity of the gradient-based
               procedure used to optimize the poisoning points (a.k.a.
               adversarial training examples). In this work, we first extend
               the definition of poisoning attacks to multiclass problems. We
               then propose a novel poisoning algorithm based on the idea of
               back-gradient optimization, i.e., to compute the gradient of
               interest through automatic differentiation, while also reversing
               the learning procedure to drastically reduce the attack
               complexity. Compared to current poisoning strategies, our
               approach is able to target a wider class of learning algorithms,
               trained with gradient-based procedures, including neural
               networks and deep learning architectures. We empirically
               evaluate its effectiveness on several application examples,
               including spam filtering, malware detection, and handwritten
               digit recognition. We finally show that, similarly to
               adversarial test examples, adversarial training examples can
               also be transferred across different learning algorithms.",
  publisher = "Association for Computing Machinery",
  pages     = "27--38",
  series    = "AISec '17",
  month     =  nov,
  year      =  2017,
  address   = "New York, NY, USA",
  keywords  = "deep learning, adversarial examples, training data poisoning,
               adversarial machine learning",
  location  = "Dallas, Texas, USA"
}


@ARTICLE{Waskom2021-fn,
  title     = "seaborn: statistical data visualization",
  author    = "Waskom, Michael",
  journal   = "J. Open Source Softw.",
  publisher = "The Open Journal",
  volume    =  6,
  number    =  60,
  pages     = "3021",
  month     =  apr,
  year      =  2021,
  copyright = "http://creativecommons.org/licenses/by/4.0/"
}

@ARTICLE{Hunter2007-el,
  title    = "Matplotlib: A {2D} Graphics Environment",
  author   = "{Hunter}",
  abstract = "Matplotlib is a 2D graphics package for Python for application
              development, interactive scripting, and publication-quality image
              generation across user interfaces and operating systems.",
  volume   =  9,
  pages    = "90--95",
  month    =  may,
  year     =  2007
}


@ARTICLE{Finlayson2019-ec,
  title    = "Adversarial attacks on medical machine learning",
  author   = "Finlayson, Samuel G and Bowers, John D and Ito, Joichi and
              Zittrain, Jonathan L and Beam, Andrew L and Kohane, Isaac S",
  journal  = "Science",
  volume   =  363,
  number   =  6433,
  pages    = "1287--1289",
  month    =  mar,
  year     =  2019,
  language = "en"
}

@ARTICLE{Finlayson2018,
  title    = "Adversarial Attacks Against Medical Deep Learning Systems",
  author   = "Finlayson, Samuel G and Chung, Hyung Won and Kohane, Isaac S and
              Beam, Andrew L",
  month         =  apr,
  year          =  2018,
  journal       = "arXiv preprint arXiv:1804.05296"
}

@ARTICLE{Matsuo2021-au,
  title     = "Backdoor Attacks to Deep Neural {Network-Based} System for
               {COVID-19} Detection from Chest X-ray Images",
  author    = "Matsuo, Yuki and Takemoto, Kazuhiro",
  abstract  = "Open-source deep neural networks (DNNs) for medical imaging are
               significant in emergent situations, such as during the pandemic
               of the 2019 novel coronavirus disease (COVID-19), since they
               accelerate the development of high-performance DNN-based
               systems. However, adversarial attacks are not negligible during
               open-source development. Since DNNs are used as computer-aided
               systems for COVID-19 screening from radiography images, we
               investigated the vulnerability of the COVID-Net model, a
               representative open-source DNN for COVID-19 detection from chest
               X-ray images to backdoor attacks that modify DNN models and
               cause their misclassification when a specific trigger input is
               added. The results showed that backdoors for both non-targeted
               attacks, for which DNNs classify inputs into incorrect labels,
               and targeted attacks, for which DNNs classify inputs into a
               specific target class, could be established in the COVID-Net
               model using a small trigger and small fraction of training data.
               Moreover, the backdoors were effective for models fine-tuned
               from the backdoored COVID-Net models, although the performance
               of non-targeted attacks was limited. This indicated that
               backdoored models could be spread via fine-tuning (thereby
               becoming a significant security threat). The findings showed
               that emphasis is required on open-source development and
               practical applications of DNNs for COVID-19 detection.",
  journal   = "NATO Adv. Sci. Inst. Ser. E Appl. Sci.",
  publisher = "Multidisciplinary Digital Publishing Institute",
  volume    =  11,
  number    =  20,
  pages     = "9556",
  month     =  oct,
  year      =  2021,
  language  = "en"
}

@ARTICLE{Feng2021-sd,
  title         = "{FIBA}: {Frequency-Injection} based Backdoor Attack in
                   Medical Image Analysis",
  author        = "Feng, Yu and Ma, Benteng and Zhang, Jing and Zhao, Shanshan
                   and Xia, Yong and Tao, Dacheng",
  abstract      = "In recent years, the security of AI systems has drawn
                   increasing research attention, especially in the medical
                   imaging realm. To develop a secure medical image analysis
                   (MIA) system, it is a must to study possible backdoor
                   attacks (BAs), which can embed hidden malicious behaviors
                   into the system. However, designing a unified BA method that
                   can be applied to various MIA systems is challenging due to
                   the diversity of imaging modalities (e.g., X-Ray, CT, and
                   MRI) and analysis tasks (e.g., classification, detection,
                   and segmentation). Most existing BA methods are designed to
                   attack natural image classification models, which apply
                   spatial triggers to training images and inevitably corrupt
                   the semantics of poisoned pixels, leading to the failures of
                   attacking dense prediction models. To address this issue, we
                   propose a novel Frequency-Injection based Backdoor Attack
                   method (FIBA) that is capable of delivering attacks in
                   various MIA tasks. Specifically, FIBA leverages a trigger
                   function in the frequency domain that can inject the
                   low-frequency information of a trigger image into the
                   poisoned image by linearly combining the spectral amplitude
                   of both images. Since it preserves the semantics of the
                   poisoned image pixels, FIBA can perform attacks on both
                   classification and dense prediction models. Experiments on
                   three benchmarks in MIA (i.e., ISIC-2019 for skin lesion
                   classification, KiTS-19 for kidney tumor segmentation, and
                   EAD-2019 for endoscopic artifact detection), validate the
                   effectiveness of FIBA and its superiority over
                   state-of-the-art methods in attacking MIA models as well as
                   bypassing backdoor defense. The code will be available at
                   https://github.com/HazardFY/FIBA.",
  month         =  dec,
  year          =  2021,
  journal       = {arXiv preprint arXiv:2112.01148}
}

@ARTICLE{Nwadike2020-gn,
  title         = "Explainability Matters: Backdoor Attacks on Medical Imaging",
  author        = "Nwadike, Munachiso and Miyawaki, Takumi and Sarkar, Esha and
                   Maniatakos, Michail and Shamout, Farah",
  abstract      = "Deep neural networks have been shown to be vulnerable to
                   backdoor attacks, which could be easily introduced to the
                   training set prior to model training. Recent work has
                   focused on investigating backdoor attacks on natural images
                   or toy datasets. Consequently, the exact impact of backdoors
                   is not yet fully understood in complex real-world
                   applications, such as in medical imaging where misdiagnosis
                   can be very costly. In this paper, we explore the impact of
                   backdoor attacks on a multi-label disease classification
                   task using chest radiography, with the assumption that the
                   attacker can manipulate the training dataset to execute the
                   attack. Extensive evaluation of a state-of-the-art
                   architecture demonstrates that by introducing images with
                   few-pixel perturbations into the training set, an attacker
                   can execute the backdoor successfully without having to be
                   involved with the training procedure. A simple 3$\times$3
                   pixel trigger can achieve up to 1.00 Area Under the Receiver
                   Operating Characteristic (AUROC) curve on the set of
                   infected images. In the set of clean images, the backdoored
                   neural network could still achieve up to 0.85 AUROC,
                   highlighting the stealthiness of the attack. As the use of
                   deep learning based diagnostic systems proliferates in
                   clinical practice, we also show how explainability is
                   indispensable in this context, as it can identify spatially
                   localized backdoors in inference time.",
  month         =  dec,
  year          =  2020,
  journal       = {arXiv preprint arXiv:2101.00008}
}


@INPROCEEDINGS{Demontis2019-oy,
  title     = "Why do adversarial attacks transfer? Explaining transferability
               of evasion and poisoning attacks",
  booktitle = "28th {USENIX} Security Symposium ({USENIX} Security 19)",
  author    = "Demontis, Ambra and Melis, Marco and Pintor, Maura and
               Jagielski, Matthew and Biggio, Battista and Oprea, Alina and
               Nita-Rotaru, Cristina and Roli, Fabio",
  pages     = "321--338",
  year      =  2019
}


@MISC{Halchenko2021-zl,
  title   = "{DataLad}: distributed system for joint management of code, data,
             and their relationship",
  author  = "Halchenko, Yaroslav and Meyer, Kyle and Poldrack, Benjamin and
             Solanky, Debanjum and Wagner, Adina and Gors, Jason and
             MacFarlane, Dave and Pustina, Dorian and Sochat, Vanessa and
             Ghosh, Satrajit and M{\"o}nch, Christian and Markiewicz,
             Christopher and Waite, Laura and Shlyakhter, Ilya and de la Vega,
             Alejandro and Hayashi, Soichi and H{\"a}usler, Christian and
             Poline, Jean-Baptiste and Kadelka, Tobias and Skyt{\'e}n, Kusti
             and Jarecka, Dorota and Kennedy, David and Strauss, Ted and
             Cieslak, Matt and Vavra, Peter and Ioanas, Horea-Ioan and
             Schneider, Robin and Pfl{\"u}ger, Mika and Haxby, James and
             Eickhoff, Simon and Hanke, Michael",
  journal = "Journal of Open Source Software",
  volume  =  6,
  number  =  63,
  pages   = "3262",
  year    =  2021
}


@ARTICLE{Bik2016-ud,
  title    = "The Prevalence of Inappropriate Image Duplication in Biomedical
              Research Publications",
  author   = "Bik, Elisabeth M and Casadevall, Arturo and Fang, Ferric C",
  abstract = "Inaccurate data in scientific papers can result from honest error
              or intentional falsification. This study attempted to determine
              the percentage of published papers that contain inappropriate
              image duplication, a specific type of inaccurate data. The images
              from a total of 20,621 papers published in 40 scientific journals
              from 1995 to 2014 were visually screened. Overall, 3.8\% of
              published papers contained problematic figures, with at least
              half exhibiting features suggestive of deliberate manipulation.
              The prevalence of papers with problematic images has risen
              markedly during the past decade. Additional papers written by
              authors of papers with problematic images had an increased
              likelihood of containing problematic images as well. As this
              analysis focused only on one type of data, it is likely that the
              actual prevalence of inaccurate data in the published literature
              is higher. The marked variation in the frequency of problematic
              images among journals suggests that journal practices, such as
              prepublication image screening, influence the quality of the
              scientific literature.",
  journal  = "MBio",
  volume   =  7,
  number   =  3,
  month    =  jun,
  year     =  2016,
  language = "en"
}


@ARTICLE{Al-Marzouki2005-jb,
  title    = "Are these data real? Statistical methods for the detection of
              data fabrication in clinical trials",
  author   = "Al-Marzouki, Sanaa and Evans, Stephen and Marshall, Tom and
              Roberts, Ian",
  abstract = "OBJECTIVES: To test the application of statistical methods to
              detect data fabrication in a clinical trial. SETTING: Data from
              two clinical trials: a trial of a dietary intervention for
              cardiovascular disease and a trial of a drug intervention for the
              same problem. OUTCOME MEASURES: Baseline comparisons of means and
              variances of cardiovascular risk factors; digit preference
              overall and its pattern by group. RESULTS: In the dietary
              intervention trial, variances for 16 of the 22 variables
              available at baseline were significantly different, and 10
              significant differences were seen in means for these variables.
              Some of these P values were extraordinarily small. Distributions
              of the final recorded digit were significantly different between
              the intervention and the control group at baseline for 14/22
              variables in the dietary trial. In the drug trial, only five
              variables were available, and no significant differences between
              the groups for baseline values in means or variances or digit
              preference were seen. CONCLUSIONS: Several statistical features
              of the data from the dietary trial are so strongly suggestive of
              data fabrication that no other explanation is likely.",
  journal  = "BMJ",
  volume   =  331,
  number   =  7511,
  pages    = "267--270",
  month    =  jul,
  year     =  2005,
  keywords = "Biomedical and Behavioral Research; Empirical Approach",
  language = "en"
}


@ARTICLE{Cina2022-of,
  title         = "Wild Patterns Reloaded: A Survey of Machine Learning
                   Security against Training Data Poisoning",
  author        = "Cin{\`a}, Antonio Emanuele and Grosse, Kathrin and Demontis,
                   Ambra and Vascon, Sebastiano and Zellinger, Werner and
                   Moser, Bernhard A and Oprea, Alina and Biggio, Battista and
                   Pelillo, Marcello and Roli, Fabio",
  abstract      = "The success of machine learning is fueled by the increasing
                   availability of computing power and large training datasets.
                   The training data is used to learn new models or update
                   existing ones, assuming that it is sufficiently
                   representative of the data that will be encountered at test
                   time. This assumption is challenged by the threat of
                   poisoning, an attack that manipulates the training data to
                   compromise the model's performance at test time. Although
                   poisoning has been acknowledged as a relevant threat in
                   industry applications, and a variety of different attacks
                   and defenses have been proposed so far, a complete
                   systematization and critical review of the field is still
                   missing. In this survey, we provide a comprehensive
                   systematization of poisoning attacks and defenses in machine
                   learning, reviewing more than 200 papers published in the
                   field in the last 15 years. We start by categorizing the
                   current threat models and attacks, and then organize
                   existing defenses accordingly. While we focus mostly on
                   computer-vision applications, we argue that our
                   systematization also encompasses state-of-the-art attacks
                   and defenses for other data modalities. Finally, we discuss
                   existing resources for research in poisoning, and shed light
                   on the current limitations and open research questions in
                   this research field.",
  month         =  may,
  year          =  2022,
  archivePrefix = "arXiv",
  primaryClass  = "cs.LG",
  eprint        = "2205.01992"
}


@ARTICLE{Marek2022-iu,
  title    = "Publisher Correction: Reproducible brain-wide association studies
              require thousands of individuals",
  author   = "Marek, Scott and Tervo-Clemmens, Brenden and Calabro, Finnegan J
              and Montez, David F and Kay, Benjamin P and Hatoum, Alexander S
              and Donohue, Meghan Rose and Foran, William and Miller, Ryland L
              and Hendrickson, Timothy J and Malone, Stephen M and Kandala,
              Sridhar and Feczko, Eric and Miranda-Dominguez, Oscar and Graham,
              Alice M and Earl, Eric A and Perrone, Anders J and Cordova,
              Michaela and Doyle, Olivia and Moore, Lucille A and Conan,
              Gregory M and Uriarte, Johnny and Snider, Kathy and Lynch,
              Benjamin J and Wilgenbusch, James C and Pengo, Thomas and Tam,
              Angela and Chen, Jianzhong and Newbold, Dillan J and Zheng, Annie
              and Seider, Nicole A and Van, Andrew N and Metoki, Athanasia and
              Chauvin, Roselyne J and Laumann, Timothy O and Greene, Deanna J
              and Petersen, Steven E and Garavan, Hugh and Thompson, Wesley K
              and Nichols, Thomas E and Yeo, B T Thomas and Barch, Deanna M and
              Luna, Beatriz and Fair, Damien A and Dosenbach, Nico U F",
  journal  = "Nature",
  volume   =  605,
  number   =  7911,
  pages    = "E11",
  month    =  may,
  year     =  2022,
  language = "en"
}


==> methods.tex <==
The enhancement attacks described in the remainder of this paper are heavily motivated by poisoning attacks, but they are distinct in both intention and attack capabilities. In poisoning attacks, particularly indiscriminate poisoning attacks, the attacker's goal is to decrease the accuracy of all test samples by adding a small number of crafted training examples \cite{Cina2022-of}. Despite the critical implications of poisoning attacks to real-world applications of machine learning, their importance in research-based machine learning is limited. A researcher would never want to manipulate data to make their model perform poorly. Enhancement attacks are based on a much more likely motivation behind manipulating data in research, which is to improve the performance of a model falsely. 

Along with differences in motivation, the capabilities of the attackers in enhancement attacks are much greater than in poisoning attacks. In most studies of poisoning attacks, attackers are assumed to be capable of \textit{adding} a small subset of points to the training data. In contrast, enhancement attackers can \textit{modify} existing points. Moreover, poisoning attackers may have complete (``white-box") or limited (``black-box" or ``gray-box") knowledge of the dataset and/or model \cite{Biggio2018-ka}. In the research setting of enhancement attacks, the attacker has even greater knowledge than the traditional ``white-box" setting, as they can modify the entire dataset, which may include both training and test data in the case of most within-dataset predictions. They can then publicly release this dataset such that the highly-performing model is computationally reproduced by others. 

In the following sections, we considered two separate attacker goals: falsely enhancing 1) overall classifier performance, and 2) performance of one method over another.


\subsubsection{GOAL \#1: Gradient-based enhancement}
\label{section:goal1}

Falsely enhancing model performance for a particular dataset is the primary situation in which enhancement may occur. The motivation for studying the feasibility of within-dataset enhancement of machine learning comes from data manipulations in non-machine learning biomedical research. For instance, about 2\% of papers investigated by \cite{Bik2016-ud} contained evidence of deliberate manipulations in biological images (e.g., western blots). However, possibilities of manipulations have not been studied for machine learning. In a hypothetical scenario, a biomedical researcher may enhance their dataset to improve prediction performance, thus leading to results that seem more impressive and interesting. The same researcher may then share this enhanced dataset, and others would computationally reproduce similar results, without any knowledge of the data manipulations that occurred. 

The key idea behind gradient-based enhancement is to ``push" the samples in the direction of a learned model to make the decision boundaries clearer and more consistent across all samples, thus improving performance. For a single held-out point, one may optimally change the classification by perturbing the point in the direction of $\nabla_xA$, where $A$ can be a decision function or loss function. For example, in the case of linear support vector machine (SVM) or logistic regression (LR):
\begin{equation}
X_{held-out, y=-1} \gets X_{held-out, y=-1} - \epsilon*w
\label{eq:adv_grad_neg}
\end{equation}
\begin{equation}
X_{held-out, y=1} \gets X_{held-out, y=1} + \epsilon*w
\label{eq:adv_grad_pos}
\end{equation}
where $w$ is a vector of model coefficients and $\epsilon$ is a scaling factor. Equations \ref{eq:adv_grad_neg}-\ref{eq:adv_grad_pos} would move the corresponding held-out points toward the correct side of the decision boundary. 
As summarized in Algorithm \ref{alg.model-based}, first a model $f$ is trained by holding one or numerous points out with K-fold partitioning. Then, the held-out point(s) are updated with $\nabla_xA$, which is the attacker gradient, such that the model will predict them correctly, and this process repeats until all points are held out. Since learned model coefficients should be similar when only holding out a small fraction of the points, this method should push all points of a given class in a consistent direction. Eventually, when the enhanced dataset is released, an independent researcher would not notice any perturbations in the dataset but would falsely find higher performance. 

\begin{algorithm}[t!]
\centering
\caption{Gradient-based enhancement attacks}\label{alg:model-enhance}
\begin{algorithmic}
\State $D \in\{X, y\}$: dataset
\State $f$: model
\State $n_{folds}$: folds for K-fold partitioning
\State $\lambda$: enhancement step size
\For{$k = 1 : n_{folds}$}
    \State Establish $D_{tr}, D_{held-out}$
    \State Train $f$
    \State $X_{held-out} \gets X_{held-out}  - \lambda \nabla_{x}A$ where $A=L(f, x)$ or $DF(f, x)$ 
\EndFor
\end{algorithmic}
\label{alg.model-based}
\end{algorithm}

\subsubsection{GOAL \#2: Enhancement of a particular method}
\label{section:goal2}
The motivation behind method enhancement would be to release a dataset and corresponding paper for which a neural network, for example, outperforms a simpler linear method. A second motivation could be for a company to demonstrate how their method (falsely) outperforms other methods to increase the valuation of a startup. Since a significant portion of biomedical machine learning research focuses on methods development, understanding the extent to which performance of one method can be enhanced over another is crucial.

A roadblock to method-specific enhancement is that the gradients used in Equations \ref{eq:adv_grad_neg}-\ref{eq:adv_grad_pos} generally transfer well across model types \cite{Demontis2019-oy}, which would make this process ineffective in enhancing performance of a specific method over another. 
Transferability of attacks from a base classifier $f_1$ to another classifier $f_2$ is defined by \cite{Demontis2019-oy} as how well an attack designed for $f_1$ works on $f_2$.  % $T=L(f_2, x+g_1, y)$, where $g_1=\nabla_xA(f_1,x)$. 
In this case, we do \textit{not} wish for the attacks to transfer between models. We want to find a new direction $g_1^\prime$ that enhances performance of $f_1$ but does not affect $f_2$. We achieve this by taking the component of $g_1$ that is orthogonal to $g_2$:
\begin{equation}
g_1^\prime = proj_{g_{2}^{\bot}}(g_1)
\label{eq:model_based_proj}
\end{equation}
Furthermore, Equation \ref{eq:model_based_proj} may not be sufficient to limit the performance of $f_2$, since $f_2$ can learn a new decision boundary after retraining. As such, we propose to include a term $g_2^\prime$ to suppress performance of $f_2$:
\begin{equation}
g_2^\prime = proj_{g_{1}^{\bot}}(g_2)
\label{eq:suppression_proj}
\end{equation}
Then, for a held-out sample, we can update it as follows to attempt to improve performance of $f_1$ but not $f_2$:
\begin{equation}
x^\prime = x - \lambda(g_1^\prime - \eta g_2^\prime)
\label{eq:model_based_update}
\end{equation}
where $\lambda$ and the suppression coefficient $\eta$ control the influence of $g_1^\prime$ and $g_2^\prime$.

Similar to the model-based data enhancement, we split the data into $k$ folds. For each partitioning, we train two models: 1) A model that we want to enhance (i.e., $f_1$), and 2) a second model that we do not want to enhance (i.e., $f_2$). 
Subsequently, Equations \ref{eq:model_based_proj}-\ref{eq:model_based_update} are applied to update the held-out data, and the process is repeated until each sample is held out once.

\begin{algorithm}[t!]
\centering
\caption{Method enhancement}\label{alg:method-enhance}
\begin{algorithmic}
\State $D \in\{X, y\}$: dataset
\State $D_e$: enhanced dataset
\State $f_1$: model to enhance
\State $f_2$: model to avoid enhancement
\State $n_{folds}$: number of folds for K-fold partitioning
\State $\lambda$: enhancement step size
\For{$k=1 : n_{folds}$}
    \State Establish $D_{train}, D_{held-out}$
    % \State \javid{Sample $X^{test}$ from $D_k^{test}$}
    \State Train $f_1, f_2$
    \State $g_1 \gets \nabla_{x}A(f_1, X_{held-out})$
    \State $g_2 \gets \nabla_{x}A(f_2, X_{held-out})$
    
    \State $X_{held-out} \gets X_{held-out}   - \lambda ( proj_{g_{2}^{\bot}}(g_1) - \eta \ proj_{g_{1}^{\bot}}(g_2) )$
    \State Update $D_{e}$ with new $X_{held-out}$
\EndFor
\end{algorithmic}
\end{algorithm}


